Variable selection in high-dimensional logistic regression models using a whitening approach

In bioinformatics, the rapid development of sequencing technology has enabled us to collect an increasing amount of omics data. Classification based on omics data is one of the central problems in biomedical research. However, omics data usually has a limited sample size but high feature dimensions, and it is assumed that only a few features (biomarkers) are active, i.e. informative to discriminate between different categories (cancer subtypes, responder/non-responder to treatment, for example). Identifying active biomarkers for classification has therefore become fundamental for omics data analysis. Focusing on binary classification, we propose an innovative feature selection method aiming at dealing with the high correlations between the biomarkers. Various research has shown the notorious influence of correlated biomarkers and the difficulty of accurately identifying active ones. Our method, WLogit, consists in whitening the design matrix to remove the correlations between biomarkers, then using a penalized criterion adapted to the logistic regression model to select features. The performance of WLogit is assessed using synthetic data in several scenarios and compared with other approaches. The results suggest that WLogit can identify almost all active biomarkers even in the cases where the biomarkers are highly correlated, while the other methods fail, which consequently leads to higher classification accuracy. The performance is also evaluated on the classification of two Lymphoma subtypes, and the obtained classifier also outperformed other methods. Our method is implemented in the \texttt{WLogit} R package available from the Comprehensive R Archive Network (CRAN).

==> Theory.tex <==
\section{Proof}
\begin{thm}
Suppose that
\begin{equation}\label{eq:IC}
    \norm{Q_{S^{c}S}^{n}(Q_{SS}^{n})^{-1}}\leq 1-\epsilon
\end{equation}
for some $\epsilon\in (0,1]$. Assume that $\lambda_{n}\rightarrow 0$ is chosen that $\lambda_{n}^{2}n-log(p)\rightarrow+\infty$ and $\lambda_{n}d\rightarrow 0$. Then $\mathbb{P}(sign(\widehat{\bbeta})=sign(\bbeta))=1-O(exp(-cn^{\gamma}))$ for some $\gamma>0$.
\end{thm}

We define a constructive procedure for generating a primal vector $\widehat{\bbeta}\in \mathbb{R}^{p}$ as well as a corresponding subgradient $\widehat{\bz}\in \mathbb{R}^{p}$ that together satisfy the zero-subgradient optimality conditions associated with the convex program (\ref{eq:est_lm}). The true support is correctly recovered if and only if the pair $(\widehat{\bbeta},\widehat{\bz})$ satisfies the following four conditions:
\begin{enumerate}[(a)]
    \item $\widehat{\bbeta}_{S^{c}}=0$
    \item $|\widehat{\bbeta}_{t}|>0$ for all $t\in S$
    \item $\widehat{\bz}_{S}=sign(\bbeta_{S}^{*})$
    \item $|\widehat{\bz}_{S^{c}}|_{\infty}<1$
\end{enumerate}
The first step in our construction is to choose the pair $(\widehat{\bbeta},\widehat{\bz})$ such that both condition (a) and (c) hold. The remainder of the analysis is then devoted to establishing that properties (b) and (d) hold with high probability.\\

We first establish a consistency result when the IC is imposed on the sample Fisher information $Q^{n}$. The remaining analysis, deferred to the full-length version, establishes that the incoherence assumption on the population version ensures that the sample version also obeys the property with probability converging to one exponentially fast.\\

\textit{Proof:} With the probability $p(X^{(i)})$ defined in (\ref{prob_log}), the gradient and Hessian of the negative log likelihood can be written as:

$$\nabla_{\bbeta} l(\bbeta)=\frac{1}{n}\sum_{i=1}^{n}p(X^{(i)})X^{(i)}-(\frac{1}{n}\sum_{i=1}^{n}y_{i}X^{(i)})\bbeta$$

$$\nabla_{\bbeta}^{2} l(\bbeta)=\frac{1}{n}\sum_{i=1}^{n}p(X^{(i)})(1-p(X^{(i)}))X^{(i)}{}^{T}X^{(i)}$$
and we note $Q(\bbeta)=\nabla^{2} l(\bbeta)$ in the following for ease of notation.
Let us also introduce the notation
$$W^{n}:=\frac{1}{n}\sum_{i=1}^{n}X^{(i)}\left(y_{i}-\frac{e^{X^{(i)}\bbeta}}{1+e^{X^{(i)}\bbeta}}\right).$$
The optimal of the problem (\ref{eq:est_lm}) must satisfy:
\begin{equation}\label{partial_lm}
    \nabla_{\bbeta} l(\widehat{\bbeta})+\lambda\widehat{\bz}=0
\end{equation}
Substituting into the subgradient optimality condition (\ref{partial_lm}) yields the equivalent condition
\begin{equation}
    \nabla l(\widehat{\bbeta})-\nabla l(\bbeta)-W^{n}+\lambda_{n}\widehat{\bz}=0.
\end{equation}
By a Taylor series expansion, this condition can be re-written as:
\begin{equation}\label{eq:subgradient}
    \nabla^{2} l(\bbeta^{*})[\widehat{\bbeta}-\bbeta^{*}]=W^{n}-\lambda_{n}\widehat{\bz}+R^{n},
\end{equation}
where the remainder $R^{n}$ is a term of order $\norm{R^{n}}_{2}=O\left(\norm{\widehat{\bbeta}-\bbeta^{*}}^{2}\right)$.\\
Using the shorthand $Q^{n}=\nabla^{2} l(\bbeta^{*})$, we write the zero-subgradient condition (\ref{eq:subgradient}) in block form as:

\begin{align}\label{eq:subgradient_new}
    Q_{S^{c}S}^{n}[\widehat{\bbeta}_{S}-\bbeta^{*}_{S}]&=W^{n}_{S^{c}}-\lambda_{n}\widehat{\bz}_{S^{c}}+R^{n}_{S^{c}},\\
     Q_{SS}^{n}[\widehat{\bbeta}_{S}-\bbeta^{*}_{S}]&=W^{n}_{S}-\lambda_{n}\widehat{\bz}_{S}+ R^{n}_{S}.
\end{align}
    
It can be shown that the matrix $Q_{SS}^{n}$ is invertible w.p. one, so that these conditions can be rewritten as
\begin{equation}
    Q_{S^{c}S}^{n}(Q_{SS}^{n})^{-1}[W_{S}^{n}-\lambda_{n}\widehat{\bz}_{S}+R_{S}^{n}]=W_{S^{c}}^{n}-\lambda_{n}\widehat{\bz}_{S^{c}}+R_{S^{c}}^{n}
\end{equation}
Re-arranging yields the condition
\begin{equation}
    Q_{S^{c}S}^{n}(Q_{SS}^{n})^{-1}[W_{S}^{n}-R_{S}^{n}]-[W_{S^{c}}^{n}-R_{S^{c}}^{n}]+\lambda_{n}Q_{S^{c}S}^{n}(Q_{SS}^{n})^{-1}\widehat{\bz}_{S}=\lambda_{n}\widehat{\bz}_{S^{c}}.
\end{equation}

\textbf{Analysis of condition (d):} We now demonstrate that $\norm{\widehat{\bz}_{S^{c}}}<1$. Using triangle inequality and the sample incoherence bound (\ref{eq:IC}) we have that:
\begin{equation}\label{eq:boundz}
    \norm{\widehat{\bz}_{S^{c}}}\leq \frac{(2-\epsilon)}{\lambda_{n}}[\norm{W^{n}}_{\infty}+\norm{R^{n}}_{\infty}]+(1-\epsilon)
\end{equation}

We complete the proof that $\norm{\widehat{\bz}_{S^{c}}}<1$ with the following two lemmas, provided in the full-length version.

\begin{lemma}
If $n\lambda_{n}-log(p)\rightarrow +\infty$, then
$$p(\frac{2-\epsilon}{\lambda_{n}}\norm{W^{n}}_{\infty}\geq\frac{\epsilon}{4})\rightarrow0$$
at rate $O(exp(-n\lambda_{n}+log(p)))$.
\end{lemma}

\begin{lemma}
If $n\lambda_{n}-log(p)\rightarrow +\infty$ and $d\lambda_{n}\rightarrow0$, then we have
$$p(\frac{2-\epsilon}{\lambda_{n}}\norm{R^{n}}_{\infty}\geq\frac{\epsilon}{4})\rightarrow0$$
at rate $O(exp(-n\lambda_{n}+log(p)))$.
\end{lemma}

We apply those two lemmas to the bound (\ref{eq:boundz}) to obtain that with probability converging to one at rate $O(exp\{exp(n\lambda_{n}^{2}-log(p))\})$, we have:
$$\norm{\widehat{\bz}_{S^{c}}}\leq \frac{\epsilon}{4}+\frac{\epsilon}{4}+(1-\epsilon)=1-\frac{\epsilon}{2}.$$

\textbf{Analysis of condition (b):} We next show that condition (b) can be satisfied, so that $sgn(\widehat{\bbeta}_{S})=sgn(\bbeta^{*}_{S})$. Define $\rho_{n}:=min_{i\in S}|\bbeta^{*}_{S}|$. From equation (\ref{eq:subgradient}) we have
\begin{equation}
    \widehat{\bbeta}_{S}=\bbeta^{*}_{S}-(Q^{n}_{SS})^{-1}[W_{S}-\lambda_{n}\widehat{\bz}_{S}+R_{S}].
\end{equation}

Therefore, in order to establish that $|\widehat{\bbeta}_{i}|>0$ for all $i\in S$, and moreover that  $sgn(\widehat{\bbeta}_{S})=sgn(\bbeta^{*}_{S})$, it suffices to show that 

$$\norm{(Q^{n}_{SS})^{-1}[W_{S}-\lambda_{n}\widehat{\bz}_{S}+R_{S}]}_{\infty}\leq \frac{\rho_{n}}{2}.$$
Using our eigenvalue bounds, we have:

\begin{align*}
    \norm{(Q^{n}_{SS})^{-1}[W_{S}-\lambda_{n}\widehat{\bz}_{S}+R_{S}]}_{\infty}&\leq \norm{(Q^{n}_{SS})^{-1}}_{\infty}[\norm{W_{S}}_{\infty}+\lambda_{n}+\norm{R_{S}}_{\infty}]\\
    &\leq \sqrt{d}\norm{(Q^{n}_{SS})^{-1}}_{2}[\norm{W_{S}}_{\infty}+\lambda_{n}+\norm{R_{S}}_{\infty}]\\
    &\leq \frac{\sqrt{d}}{C_{min}}[\norm{W_{S}}_{\infty}+\lambda_{n}+\norm{R_{S}}_{\infty}].
\end{align*}

In fact, the righthand side tends to zero from our earlier results on $W$ and $R$, and the assumption that $\lambda_{n}d\rightarrow0$. Together with the exponential rates of convergence established by the state lemmas, this complete the proof of the result.



==> intro.tex <==
\textcolor{blue}{je n'aime pas trop ton début, je n'aime que tu écrives des probabilités conditionnelles partout sinon il faudrait écrire des vraisemblances conditionnelles ce que tu ne fais pas. Je n'aime pas trop tes notations. Je ne vois pas l'intérêt d'expliquer la méthode de Newton, il faut commencer tout de suite en disant qu'on veut estimer les beta
  dans un contexte sparse. 
Par ailleurs, tout ce début doit aller en introduction pas dans la partie ``Methods''.}

\textcolor{blue}{
  Je pense qu'il faut commencer l'intro en expliquant pourquoi c'est important de faire de la sélection de variables dans un contexte de réponse binaire dans le
  domaine médical qui intéresse Sanofi. Ensuite dire qu'une façon naturelle de faire ça c'est de faire de la vraisemblance pénalisée et de montrer que l'on peut
  en faisant un développement de Taylor à l'ordre 2 approcher la log-vraisemblance par $\ell_Q$. Ca c'est pour la structure du début du papier.
  Après je suis embêtée par ton critère d'irreprésentabilité parce qu'en fait il n'est pas du tout justifier à part de dire : on espère que ça va se passer comme dans le modèle linéaire classique.... Pour le critère d'irreprésentabilité je suis gênée aussi par le fait que tu l'écrives avec une espérance parce qu'en fait dans ton modèle tu tires les X une fois et ensuite ils sont fixés donc c'est un peu bizarre....
}

\textcolor{blue}{
Let $x_{i,k}$ denote the $i$th observation of the $k$th predictor. Assume moreover that $Y_1,Y_2,...,Y_n$ are independent random variables having a Bernoulli distribution such that $Y_i\sim\textrm{Bernoulli}(\pi_{\bbeta}(\bx_i))$ where for all $i$ in $\{1,\dots,n\}$,
$$
\pi_{\bbeta}(\bx_i)=\frac{\exp\left({\sum_{k=1}^p \beta_k x_{i,k}}\right)}{1+\exp\left({\sum_{k=1}^p \beta_k x_{i,k}}\right)},
$$
with $\bx_{i}=(x_{i,1},\dots,x_{i,p})$.
}

%%% Local Variables:
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "main_CLL"
%%% ispell-local-dictionary: "en_US"
%%% eval: (flyspell-mode 1)
%%% End:
